Optimization methods for MR image reconstruction (long version)

The development of compressed sensing methods for magnetic resonance (MR) image reconstruction led to an explosion of research on models and optimization algorithms for MR imaging (MRI). Roughly 10 years after such methods first appeared in the MRI literature, the U.S. Food and Drug Administration (FDA) approved certain compressed sensing methods for commercial use, making compressed sensing a clinical success story for MRI. This review paper summarizes several key models and optimization algorithms for MR image reconstruction, including both the type of methods that have FDA approval for clinical use, as well as more recent methods being considered in the research community that use data-adaptive regularizers. Many algorithms have been devised that exploit the structure of the system model and regularizers used in MRI; this paper strives to collect such algorithms in a single survey. Many of the ideas used in optimization methods for MRI are also useful for solving other inverse problems.

==> def/def,eps.tex <==
% def,eps.tex
% Latex2e macros for including Encapsulated Postscript (.eps)
% /opt/gnu/tex/doc/user/grfguide.ps
% Needs: \usepackage[dvips,draft]{graphicx}
% Picture: \ineps{dir}{file}{size}
% Centered picture: \inceps{dir}{file}{size}
% Captioned figure: \figeps[htbp]{dir}{file}{size}{caption}
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
% Centered quad figure:
%	\figepsquad{size}{dir}{file1}{file2}{file3}{file4}{caption}
% "file" does not include the .eps, and also becomes the figure label.
% "size" is typically Esize.  optional argument specifies position
% note: the graphicx package has a command that can specify order of
% suffixes to try: \DeclareGraphicsExtensions{.eps,.pdf}
%
\ifx \ecaption \undefined
	\newcommand{\ecaption}{\caption}
\fi

%
% \inps{width=}{size}{dir}{root}{suffix}
%
\providecommand{\figcent}[1]		{\mbox{}\hfill#1\hfill\mbox{}}
%\providecommand{\figsuffix}		{.eps}
\providecommand{\figsuffix}		{}
\providecommand{\figsuffixc}		{.epsc}
\providecommand{\inps}[5]		{\includegraphics[#1#2]{#3/#4#5}}
\providecommand{\ineps}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffix}}
\providecommand{\inepsc}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffixc}}
\providecommand{\inceps}[4][width=]	{\figcent{\ineps[#1]{#2}{#3}{#4}}}
\providecommand{\inpdf}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.pdf}}
\providecommand{\injpg}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.jpg}}
\providecommand{\intga}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.tga}}
\providecommand{\flabel}[1]		{\label{#1}} % figure label

% captioned/labeled eps, for use within a multiple-plot floating figure
\providecommand{\capeps}[4]{% dir file width caption
\inceps{#1}{#2}{#3}%
\ecaption{#4}%
\flabel{#2}}

\providecommand{\figeps}[5][htbp]{%
\begin{figure}[#1]%
\capeps{#2}{#3}{#4}{#5}%
\end{figure}}

\providecommand{\figepsc}[5][htbp]{%
\begin{figure}[#1]%
\figcent{\inepsc{#2}{#3}{#4}}%
\ecaption{#5}%
\flabel{#3}%
\end{figure}}

\providecommand{\figepsstar}[5][htbp]{%
\begin{figure*}[#1]%
\inceps{#2}{#3}{#4}%
\ecaption{#5}%
\flabel{#3}%
\end{figure*}}

%
% for 2 side-by-side
%

%
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
\providecommand{\incepslr}[4]{%
\lfill\ineps{#1}{#2}{#4}\hfill\ineps{#1}{#3}{#4}\rfill}

%
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
%
\providecommand{\figepslr}[6][htbp]{%
\begin{figure}[#1]%
\incepslr{#2}{#3}{#4}{#5}%
\ecaption{#6}%
\flabel{#3}%
\flabel{#4}%
\end{figure}}

%
% captioned 4 as 2by2
%

%
% Captioned quad figure:
% \figepsquad[htbp]{size}{dir}{file1}{file2}{file3}{file4}{caption}
\providecommand{\figepsquad}[8][htbp]{%
\begin{figure}[#1]%
\incepslr{#3}{#4}{#5}{#2}%
\\%
\incepslr{#3}{#6}{#7}{#2}%
\ecaption{#8}%
\flabel{#4}\flabel{#5}\flabel{#6}\flabel{#7}%
\end{figure}}


==> def/def,gen.tex <==
% def,gen.tex
% Latex2e general macros
% Jeff Fessler

% sections
%\providecommand{\dirtex}		{/n/ir7/y/fessler/tex}
%\providecommand{\dirtex}		{.} % use TEXINPUTS instead
\providecommand{\inputtex}[1]		{\label{#1}\input{#1}}
\providecommand{\isection}[2]		{\section{#1}\inputtex{#2}}
\providecommand{\isubsection}[2]	{\subsection{#1}\inputtex{#2}}

% latin
%\providecommand{\etal}		{\emph{et al\@.}\xspace}
\providecommand{\etal}		{et al\@.\xspace}
\providecommand{\ie}		{\emph{i.e\@.}\xspace}
\providecommand{\eg}		{\emph{e.g\@.}\xspace}
\providecommand{\cf}		{\emph{cf\@.}\xspace}
\providecommand{\defacto}	{\emph{de facto}\xspace}
\providecommand{\adhoc}		{\emph{ad hoc}\xspace}
\providecommand{\apriori}	{\emph{a priori}\xspace}

% web
%\providecommand{\myurl}[1][]	{\texttt{http://web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurlold}[1][]	{\texttt{web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurl}[1][]	{\url{http://web.eecs.umich.edu/~fessler#1}\xspace}
\providecommand{\myweb}		{\url{http://web.eecs.umich.edu/~fessler}\xspace}
\providecommand{\onweb}[1]	{Available from \myweb.}


% comments environments
% when using \usepackage{verbatim},
% the following allows this: \begin{comments} ... \end{comments} 
\let\comments=\comment
\let\endcomments=\endcomment

% huge comments.
% unfortunately this bashes the \begin{comment} environment in verbatim.sty
% which is why i have defined the preceding \comments environment.
\long\def\comment#1{}
\providecommand{\uncomment}[1]	{#1}


% common environments
\providecommand{\bcent}		{\begin{center}}
\providecommand{\ecent}		{\end{center}}
\providecommand{\benum}		{\begin{enumerate}}
\providecommand{\eenum}		{\end{enumerate}}
\providecommand{\bitem}		{\begin{itemize}}
\providecommand{\eitem}		{\end{itemize}}
\providecommand{\bvers}		{\begin{verse}}
\providecommand{\evers}		{\end{verse}}
\providecommand{\btab}		{\begin{tabbing}}	% use \= and \>
\providecommand{\etab}		{\end{tabbing}}
%\providecommand{\bverb}	{\begin{verbatim}}
%\providecommand{\everb}	{\end{verbatim}}

% positioning
\providecommand{\lfill}		{\mbox{}\hfill}
\providecommand{\rfill}		{\hfill\mbox{}}
\newcommand{\cent}[1]		{\lfill{#1}\rfill}

% box with text stacked up in it
%\newcommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\DeclareRobustCommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\fsbox}[2][c]	{\fbox{\stacktext[#1]{#2}}}

\providecommand{\ul}[1]		{\underline{#1}}
\providecommand{\ebox}[1]	{\mbox{\fbox{$\displaystyle#1$}}}
\providecommand{\cbox}[1]	{\[\ebox{#1}\]}

% top-aligned side-by-side mini-pages
\newcommand{\minipagett}[4] {% width1 width2 box1 box2
\begin{minipage}[t]{#1\linewidth}\vspace*{0pt}#3\end{minipage}%
\hfill%
\begin{minipage}[t]{#2\linewidth}\vspace*{0pt}#4\end{minipage}}

% bullet list with normal spacing
\newcounter{blist}
\providecommand{\blistmark}	{\makebox[0pt]{$\bullet$}}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\blist}[1][]	{%
\begin{list}{\blistmark}{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{0.5\leftmargin}% centers label in margin
\setlength{\labelwidth}{0em}%
#1}% user over-rides
}
\providecommand{\elist}		{\end{list}}
\providecommand{\elistup}	{\elist\vspace{-\parskip}} % no space after

% enum list with normal spacing
%\providecommand{\bcolor}[1] {#1}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\bjfenum}[1][]	{%
\begin{list}{\bcolor{\arabic{blist}.} }{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{0.0em}%
\setlength{\labelsep}{1.0\leftmargin}% label in margin?
\setlength{\labelwidth}{0pt}%
#1}% user over-rides
}

% Alpha list with normal spacing
\newcounter{blistAlph}
\providecommand{\blistAlph}[1][]
{\begin{list}{\makebox[0pt][l]{\Alph{blistAlph}.}}{%
\usecounter{blistAlph}%
\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{1.0\leftmargin}% letter at left side of margin
\setlength{\labelwidth}{0.0\leftmargin}#1}%
}

% Roman list with a bit of spacing
\newcounter{blistRoman}
\providecommand{\blistRoman}[1][]
{\begin{list}{\Roman{blistRoman}.}{%
\usecounter{blistRoman}%
\setlength{\itemsep}{0.5em}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{4em}%
\setlength{\labelsep}{0.4\leftmargin}
\setlength{\labelwidth}{0.6\leftmargin}#1}%
}

%
% Portrait
% use \pagesize[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
% at top of page: 1in, \topmargin, \headheight(for header), \headsep
%
\providecommand{\myheadheight}	{0in}
\providecommand{\myheadsep}	{0in}
\providecommand{\Halfheight}	{5.5in}		% half of 11" vertical page
\providecommand{\Halfwidth}	{4.25in}	% half of 8.5" horizontal page
\providecommand{\pagesize}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{\myheadsep}
\setlength{\headheight}{\myheadheight}
\setlength{\oddsidemargin}{\Halfwidth}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{\Halfheight}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-0.5\headheight}
\addtolength{\topmargin}{-0.5\headsep}
\addtolength{\topmargin}{-1in}
}

%
% Landscape
% use \pagesizeland[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
%
\providecommand{\pagesizeland}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{0.0in}
\setlength{\headheight}{0.0in}
\setlength{\oddsidemargin}{5.5in}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{4.25in}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-1in}
}

%
% half of top margin for headings.
%
\providecommand{\pagehead}{%
\setlength{\headsep}{\topmargin}%
\addtolength{\headsep}{1in}%
\setlength{\headsep}{0.5\headsep}%
\setlength{\headheight}{\headsep}%
\setlength{\topmargin}{-1in}%
}


==> def/def,math.tex <==
% def,math.tex
% latex2e definitions of math symbols

% todo: to fix fonts see http://tug.org/fonts/fontinstall.html
%\usepackage{bbm} % black-board math
%\providecommand{\jfbbm}[1]	{\xmath{\mathbbm{#1}}} % needs bbm package
%\providecommand{\jfbbm}[1]	{\xmath{\mathsf{#1}}} % todo: while bbm broken
\providecommand{\jfbbm}[1]	{\xmath{\mathbb{#1}}}

\providecommand{\qed}[1][0pt]	{\hfill\raisebox{#1}{\inmath{\Box}}} % need latexsym package
% the next command is my favorite way to define bold letters.
% it requires \usepackage{bm,jf-fun}
\providecommand{\blmath}[1]	{\jfunl{\bm{#1}}}	% bm, jf-fun

% symbols that might need defined in a symbol table
\providecommand{\bigone}[1][\Large]	{\mbox{ {#1 1}}\xspace}
%\providecommand{\indic}[2][\large]	{\xmath{\mbox{{#1 $1$}}_{\braces{#2}}}}
% another option for \indic would be \iota
\providecommand{\indic}[2][]	{\xmath{\jfbbm{I}_{\braces{#2}}}}

%\providecommand{\reals}	{\xmath{\mathrm{I\kern-.2em R}}}
\providecommand{\reals}		{\jfbbm{R}}

\providecommand{\thus}		{\xmath{\stackrel{\textstyle .}{..}}}
\providecommand{\suchthat}	{\textnormal{ s.t. }}
\providecommand{\defequ}	{\stackrel{\bigtriangleup}{=}}
\providecommand{\iid}		{\stackrel{iid}{\sim}}
\providecommand{\icomplex}	{\xmath{\imath}}

\providecommand{\norm}[1]	{\xmath{\left\| #1 \right\|}}
\providecommand{\normb}[1]	{\xmath{\Big\| #1 \Big\|}}
\providecommand{\normbb}[1]	{\xmath{\Bigg\| #1 \Bigg\|}}
\providecommand{\floor}[1]	{\xmath{\left\lfloor #1 \right\rfloor}}
\providecommand{\ceil}[1]	{\xmath{\left\lceil #1 \right\rceil}}
%\providecommand{\inprod}[2]	{\xmath{\langle #1,\, #2 \rangle}}
\providecommand{\inprod}[2]	{\xmath{\mathop{\langle #1,\, #2 \rangle}\nolimits}}
\providecommand{\Inprod}[2]	{\xmath{\left\langle #1,\ #2 \right\rangle}}
\providecommand{\musec}		{\xmath{\mu\mathrm{sec}}}

% \modo: ordinary modulo with a bit of space: "x mod y"
\providecommand{\modo}[2]	{\xmath{#1 \mathop{\mathrm{mod}}\nolimits #2}}
% \modp: modulo with the first part in paren: "(x) mod y"
\providecommand{\modp}[2]	{\modo{(#1)}{#2}}
% \pmod: defined in amsmath to do (x mod y)


\let\equivsave\equiv
\def\equiv{\xmath{\equivsave}}

% notes
% amsmath has subscript stacking: \sum_{\substack{ n=1 \\ n \neq m}}^N
% dvips -Ppdf for making pdf files?  \special for pdf hyperlinks?

\providecommand{\sumstack}[2]	{\sum_{\substack{#1 \\ #2}}}

\providecommand{\ba}[1]		{\left[ \begin{array}{#1}}
\providecommand{\ea}		{\end{array} \right]}
\providecommand{\be}		{\begin{equation}}
\providecommand{\ee}[1]		{\label{#1}\end{equation}}
\providecommand{\den}[2]	{\begin{equation} #1 \label{#2} \end{equation}}
\providecommand{\bea}		{\begin{eqnarray}}
\providecommand{\eea}[1]	{\label{#1}\end{eqnarray}}
\providecommand{\beas}		{\begin{eqnarray*}} % obsolete! use desa{}
\providecommand{\eeas}		{\end{eqnarray*}} % obsolete!
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
%\providecommand{\eels}		{\end{align*}}
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
\providecommand{\beals}[1][1]	{\begin{alignat*}{#1}} % requires amsmath
\providecommand{\eeals}		{\end{alignat*}}

% displayed but un-numbered (*'d) equations using aligned
\providecommand{\desa}[1]	{\begin{equation*}%
	\begin{aligned}#1\end{aligned}\end{equation*}} % amsmath
% variant where first line is moved left using \MoveEqLeft from mathtools
\providecommand{\desal}[1]	{\begin{equation*}%
	\begin{aligned}\MoveEqLeft#1\end{aligned}\end{equation*}} % amsmath

% numbered versions (these number every line unless \nonum or \notag used)
\providecommand{\dena}[2]
	{\begin{align}#1\label{#2}\end{align}} % amsmath
\providecommand{\denal}[2]
	{\begin{align}\MoveEqLeft#1\label{#2}\end{align}} % amsmath

\providecommand{\denalt}[3]{ % text eqn label
\begin{flalign}
\text{#1} && #2 &&
\label{#3}
\end{flalign}
}

% obsolete: use desa and dena instead
\providecommand{\bals}		{\begin{equation*}\begin{aligned}} % amsmath
\providecommand{\eals}		{\end{aligned}\end{equation*}}
\providecommand{\beal}		{\begin{equation}\begin{aligned}[b]}
\providecommand{\eeal}[1]	{\end{aligned}\label{#1}\end{equation}}

% these do not work:
% http://tex.stackexchange.com/questions/3169/making-a-new-environment-combining-equation-and-split/3205#3205
%\providecommand{\bal}		{\begin{align}} % amsmath
%\providecommand{\eal}[1]	{\label{#1}\end{align}}
% but this works:
\providecommand{\bale}[2]	{\begin{align}#1\label{#2}\end{align}} % amsmath


% note: \ber and \eer and \bear are all dangerous it seems.
% use \berr and bearr instead!

%\providecommand{\ber}[1]	{\bgroup\renewcommand{\theequation}{#1}\be}
%\providecommand{\eer}[1]	{\label{#1}\end{equation}\egroup}
\providecommand{\berr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\be
#2
\ee{e,#1}
\egroup
\ignorespaces
}

%\providecommand{\bear}[1]	{\renewcommand{\theequation}{#1}\bea}
\providecommand{\bearr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\bea
#2
\eea{e,#1}
\egroup
\ignorespaces
}

% can this be done?
%\providecommand{\bebox}[1][\mbox{\fbox{$\displaystyle]	{\begin{equation}#1}
%\providecommand{\eebox}[1]	{$\}\}\label{#1}\end{equation}}
%\providecommand{\eebox}[2][$\}\}]	{#1\label{#2}\end{equation}}

\providecommand{\inmath}	{\ensuremath}
\providecommand{\xmath}[1]	{\inmath{#1}\xspace}
\providecommand{\bmath}[1]	{\xmath{\bm{#1}}}	% needs \usepackage{bm}
\providecommand{\eref}[1]	{(\protect\ref{#1})}
\providecommand{\fref}[2][]	{Fig.~\protect\ref{#2}#1}
\providecommand{\conj}		{\inmath{^*}}
%\providecommand{\conj}		{\inmath{^{\star}}}
\providecommand{\conjb}[1]	{\xmath{\brak{#1}\conj}} % [ ... ]^*
\providecommand{\degr}		{\xmath{^{\circ}}}
\providecommand{\isotop}[2]	{\inmath{^{#2}}#1\xspace}

\providecommand{\conv}		{\inmath{\ast}}
\providecommand{\cconv}		{\inmath{\ast\mbox{$\!\!$}\ast}}
\providecommand{\cconvsub}	{\inmath{\ast\mbox{$\!$}\ast}}
\providecommand{\ccconv}	{\inmath{\mathbin{\ast \mbox{$\!\!$} \ast \mbox{$\!\!$}\ast}}}

\providecommand{\inv}		{\inmath{^{-\!1}}}
\providecommand{\invT}		{\inmath{^{-\!\mathrm{T}}}}
\providecommand{\invH}		{\inmath{^{-\!\mathrm{H}}}}
\providecommand{\powten}[1]	{\inmath{\cdot10^{#1}}}
\providecommand{\uminus}	{\mathord{-}}

% invisible rule to make brackets etc. bigger
\providecommand{\irule}[1][-0.7em] {\rule[#1]{0pt}{0pt}}

\providecommand{\evalat}[2]	{\left. #1 \right|_{#2}}
\providecommand{\Evalat}[3][0.7em]
	{\left. #2 \irule[-#1] \right|_{#3}}	% -0.4\baselineskip
\providecommand{\choos}[3][-0.2]
% {\xmath{\fbox{\xmath{\begin{array}{c} #2\\[#1em]#3 \end{array}}}}}
 {\xmath{\left(\begin{array}{c} #2\\[#1em]#3 \end{array}\right)}}
%\providecommand{\choos}[2]	{\xmath{\left(\stackrel{#1}{#2}\right)}}

% \parin is "mathinner" parentheses; leaves more space around nearby operations
\providecommand{\parin}[1]	{\xmath{\mathinner{\left(#1\right)}}}
\providecommand{\paren}[1]	{\xmath{\left(#1\right)}}
\providecommand{\parenb}[1]	{\xmath{\Big(#1\Big)}}
\providecommand{\parens}[1]	{\xmath{(#1)}}
%\providecommand{\of}[1]	{\!\left(#1\right)}
\providecommand{\of}[1]		{\mleft(#1\mright)}
\providecommand{\ofb}[1]	{\!\Big(#1\Big)}
\providecommand{\brak}[1]	{\xmath{\left[#1\right]}}
\providecommand{\brakleft}[1]	{\xmath{\left[#1\right.}}
\providecommand{\brakright}[1]	{\xmath{\left.#1\right]}}
\providecommand{\brakb}[1]	{\xmath{\Big[#1\Big]}}
\providecommand{\brakbb}[1]	{\xmath{\Bigg[#1\Bigg]}}
\providecommand{\braces}[1]	{\xmath{\left\{#1\right\}}}
\providecommand{\bracesb}[1]	{\xmath{\Big\{#1\Big\}}}
\providecommand{\bracesbb}[1]	{\xmath{\Bigg\{#1\Bigg\}}}
\providecommand{\abs}[1]	{\xmath{\left| #1 \right|}}
\providecommand{\absb}[1]	{\xmath{\Big| #1 \Big|}}
\providecommand{\absbb}[1]	{\xmath{\Bigg| #1 \Bigg|}}

\providecommand{\overtext}[2]	{\overbrace{#1}^{\mbox{#2}}}
%\providecommand{\undertext}[2]	{\underbrace{#1}_{\mbox{#2}}}
\DeclareRobustCommand{\undertext}[2] {\underbrace{#1}_{\mbox{#2}}}
%\providecommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}
\DeclareRobustCommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}

\providecommand{\dddot}[1]	{\inmath{#1^{(3)}}}
\providecommand{\ddddot}[1]	{\inmath{#1^{(4)}}}
\providecommand{\dsqrt}[1]	{\xmath{\sqrt{\displaystyle #1}}}

\providecommand{\xfrac}[2]	{\xmath{\frac{#1}{#2}}}
\providecommand{\Half}[1][1]	{\xfrac{#1}{2}}
\providecommand{\half}[1][1]	{\xmath{{\scriptstyle \frac{#1}{2}}}}
\providecommand{\Frac}[2]	{\xmath{{#1}/{#2}}}
\providecommand{\pfrac}[3][]	{\xmath{\!\paren{#1\frac{#2}{#3}}}}
\providecommand{\pFrac}[3][]	{\xmath{\!\paren{#1\Frac{#2}{#3}}}}
\providecommand{\dpfrac}[3][]	{\xmath{\!\paren{#1\dfrac{#2}{#3}}}}
%\providecommand{\dfrac}[2]	% conflicts with amstex
\def\dfrac#1#2{\xmath{\displaystyle\frac{#1}{#2}}}
\def\implies	{\xmath{\Longrightarrow}} % ams?

%\providecommand{\eexp}		{\xmath{\mathop{\mathrm{e}}\nolimits}}
\providecommand{\eexp}		{\xmath{\mathinner{\mathrm{e}}}}
\providecommand{\Expi}[1]	{\xmath{\eexp^{\icomplex #1}}}
\providecommand{\expi}[1]	{\xmath{\exp\of{\icomplex #1}}}
\providecommand{\Expni}[1]	{\xmath{\eexp^{-\icomplex #1}}}
\providecommand{\expni}[1]	{\xmath{\exp\of{-\icomplex #1}}}
\providecommand{\Expo}[1]	{\xmath{\eexp^{#1}}}
\providecommand{\expo}[1]	{\xmath{\exp\of{#1}}}
\providecommand{\Expn}[1]	{\xmath{\eexp^{-#1}}}
\providecommand{\expn}[1]	{\xmath{\exp\of{-#1}}}
\providecommand{\Exp}		{\expo}	% backward compat
\providecommand{\Cos}[1]	{\xmath{\cos\of{#1}}}
\providecommand{\Sin}[1]	{\xmath{\sin\of{#1}}}

%
% the following are all obsolete due to jf-fun.sty
%
\providecommand{\Normal}[1]	{{\mathcal N}\of{#1}}
\providecommand{\mathword}[3][]	{\,\inmath{\mathrm{#2}#1\of{#3}}}
\providecommand{\wordbrace}[3][]{\,\inmath{\mathrm{#2}#1\!\braces{#3}}}
\providecommand{\Poisson}[1]	{\wordbrace{Poisson}{#1}}
\providecommand{\diag}[1]	{\wordbrace{diag}{#1}}
\providecommand{\var}[1]	{\wordbrace{Var}{#1}}
\providecommand{\cov}[1]	{\wordbrace{Cov}{#1}}
%\providecommand{\sinc}[2][]	{\mathword[#1]{sinc}{#2}}
\providecommand{\sinc}		{\Ofun{\mathrm{sinc}}}
\providecommand{\rect}[1] 	{\mathword{rect}{#1}}
\providecommand{\sgn}[1] 	{\mathword{sgn}{#1}}
\providecommand{\real}[1]	{\mathword{real}{#1}}
\providecommand{\imag}[1]	{\mathword{imag}{#1}}

\providecommand{\mystack}[2][c]	{\xmath{\begin{array}{#1} #2 \end{array}}}
\providecommand{\myvect}[2][c]	{\xmath{\brak{\mystack[#1]{#2}}}}
\providecommand{\mymat}[1]	{\xmath{\begin{bmatrix} #1 \end{bmatrix}}} % amsmath, up to 10 cols, does not require [ccc]
\DeclareRobustCommand{\pmymat}[1] {\xmath{\begin{bmatrix} #1 \end{bmatrix}}}
\providecommand{\mymatsmall}[1]	{\xmath{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}} % amsmath, up to 10 cols, does not require [ccc]
\providecommand{\mymato}[2][]	{\xmath{\begin{bmatrix}[#1] #2 \end{bmatrix}}}
\providecommand{\leftbrace}[2][ll]	{\left\{ \mystack[#1]{#2} \right.}
\providecommand{\zeroother}	{\\ 0, & \mathrm{otherwise}}

% integrals and derivatives
\providecommand{\negint}	{-\!\!\int\!}
\providecommand{\intinf}	{\int_{\!-\infty}^{\infty}}
\providecommand{\iintinf}	{\intinf\intinf}
\providecommand{\iint}		{\int\!\!\!\int}
\providecommand{\iiint}		{\int\!\!\!\int\!\!\!\int}
\providecommand{\iiiint}	{\int\!\!\!\int\!\!\!\int\!\!\!\int}
% caution: \der \xj_n must be \der{\xj_n} to work properly!
\providecommand{\der}[1]	{\xmath{\mathop{\mathrm{d}#1}\nolimits}}
%\providecommand{\der}		{\xmath{\mathop{\mathrm{d}}\nolimits}}
%\providecommand{\der}		{\xmath{\mathrm{d}}}
\providecommand{\dxy}		{\der{x}\der{y}}
\providecommand{\dxyz}		{\der{x}\der{y}\der{z}}

\providecommand{\ddt}[1][t]	{\xfrac{\der{}}{\der{#1}}}
\providecommand{\dder}[2]	{\xfrac{\der{}^{#2}}{\der{#1}^{#2}}}
\providecommand{\fpart}[2][]	{\xfrac{\partial #1}{\partial #2}}
\providecommand{\ffpart}[2][]	{\xfrac{\partial^2 #1}{\partial #2^2}}
\providecommand{\fffpart}[2][]	{\xfrac{\partial^3 #1}{\partial #2^3}}
\providecommand{\ffpartt}[2]	{\xfrac{\partial^2}{\partial #1 \; \partial #2}}
%\providecommand{\Part}[1]	{\frac{\partial}{\partial #1}}
%\providecommand{\Partt}[1]	{\frac{\partial^2}{\partial #1}}
%\providecommand{\Parttt}[1]	{\frac{\partial^3}{\partial #1}}

\providecommand{\Gam}		{\jfunl{\Gamma}}
\providecommand{\eps}		{\jfunl{\epsilon}}
\providecommand{\veps}		{\jfunl{\varepsilon}}

